Needle in a Haystack: Label-Efficient Evaluation under Extreme Class Imbalance

Important tasks like record linkage and extreme classification demonstrate extreme class imbalance, with 1 minority instance to every 1 million or more majority instances. Obtaining a sufficient sample of all classes, even just to achieve statistically-significant evaluation, is so challenging that most current approaches yield poor estimates or incur impractical cost. Where importance sampling has been levied against this challenge, restrictive constraints are placed on performance metrics, estimates do not come with appropriate guarantees, or evaluations cannot adapt to incoming labels. This paper develops a framework for online evaluation based on adaptive importance sampling. Given a target performance metric and model for $p(y|x)$, the framework adapts a distribution over items to label in order to maximize statistical precision. We establish strong consistency and a central limit theorem for the resulting performance estimates, and instantiate our framework with worked examples that leverage Dirichlet-tree models. Experiments demonstrate an average MSE superior to state-of-the-art on fixed label budgets.

==> subfiles/abstract.tex <==
\begin{abstract}
    Important tasks like record linkage and extreme classification 
    demonstrate extreme class imbalance, with 1 minority 
    instance to every 1 million or more majority instances. 
    Obtaining a sufficient sample of all classes, even just to achieve 
    statistically-significant evaluation, is so challenging that most current 
    approaches yield poor estimates or incur impractical cost. 
    Where importance sampling has been levied against this challenge, 
    restrictive constraints are placed on performance metrics, estimates do 
    not come with appropriate guarantees, or evaluations 
    cannot adapt to incoming labels.
    This paper develops a framework for online evaluation based 
    on adaptive importance sampling. 
    Given a target performance metric and model for $p(y|x)$, the 
    framework adapts a distribution over items to label in order to 
    maximize statistical precision. 
    We establish strong consistency and a central limit theorem for the 
    resulting performance estimates, and instantiate our framework with 
    worked examples that leverage Dirichlet-tree models.
    Experiments demonstrate an average MSE superior to state-of-the-art 
    on fixed label budgets.
\end{abstract}
    

==> subfiles/practicalities.tex <==
\subsection{Practicalities}
\label{sec:practicalities}
\comment{Move whole section to Appendix?}
\paragraph{Sample reuse.}
Suppose our framework is used to estimate a generalized 
measure $G_1$. 
If the joint distribution $p(x,y)$ associated with the prediction 
problem has not changed, it may be desirable to \emph{reuse} the 
weighted samples $\mathcal{L}$ to estimate a different generalized 
measure $G_2$. 
This is possible so long as the sequence of proposals used to estimate 
$G_1$ have the required support for $G_2$. 
More precisely, the support of $q_j(x,y)$ must include
$\{x, y \in \Xspace \times \Yspace : \|\ell(x, y)\| p(x, y) \neq 0 \}$ 
for the loss functions associated with $G_1$ \emph{and} $G_2$.

If one anticipates sample reuse, the proposals can be made 
less specialized to a particular generalized measure by mixing 
with the marginal distribution $p(x)$, i.e.\ 
$q(x) \to (1 - \delta) q(x) + \delta p(x)$
where $\delta \in (0, 1]$ is a hyperparameter that controls the 
degree of specialization.

\paragraph{Confidence region.}
\label{sec:confidence-region}
An asymptotic $100(1-\alpha)\%$ confidence region for $G$ 
is given by the ellipsoid formed by vectors $G^\star \in \reals^k$ 
such that
\begin{equation*}
  (G^\star - \hat{G})^\intercal \hat{\Sigma}^{-1} (G^\star - \hat{G}) \leq 
    \frac{(N - 1)k}{N(N - k)} F_{\alpha,k,N-k},
  \label{eqn:confidence-region}
\end{equation*}
where $\hat{G}$ is the sample mean, $\hat{\Sigma}$ is the sample 
covariance matrix, and $F_{\alpha,d_1,d_2}$ is the critical value of the 
$F$ distribution with $d_1, d_2$ degrees of freedom at significance level 
$\alpha$.

We can approximate this region using the AIS estimator for $G$ in 
\eqref{eqn:G-AIS} and the following estimator for $\Sigma$:
\begin{equation*}
  \begin{split}
    \hat{\Sigma}^{\mathrm{AIS}} = \Jac_g (\hat{R}^{\mathrm{AIS}}) &\bigg( \frac{1}{N} \sum_{j = 1}^{N} 
        \frac{p(x_j)^2 \ell(x_j, y_j) \ell(x_j, y_j)^\intercal}{q_N(x_j) q_{j-1}(x_j)} 
       - \hat{R}^{\mathrm{AIS}} \hat{R}^{\mathrm{AIS}\intercal} \bigg) \Jac_g (\hat{R}^{\mathrm{AIS}})^\intercal.
  \end{split}
\end{equation*}
This is obtained from the expression for the asymptotic covariance matrix 
$\Sigma$ in Theorem~\ref{thm:ais-clt},
% \begin{align*}
%   \Sigma = \Jac g(R) & \bigg( \underset{X,Y \sim p}{\E} 
%     \left[ \frac{p(X) \ell(X, Y) \ell(X, Y)^\intercal}{q_\infty(X)} \right] \\
%     & \qquad {} - R R^\intercal \bigg) \Jac g(R)^\intercal.
% \end{align*}
by using an AIS estimator for the variance and $R$, and approximating 
$q_\infty(x)$ by the most recent proposal $q_N(x)$.


==> subfiles/preamble.tex <==
\usepackage{xr-hyper}       % cross-referencing (must be loaded before hyperref)

% CUSTOM PACKAGES
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm, amssymb}
\usepackage{bm}             % bold math symbols
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xcolor}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{caption}
\usepackage{subcaption}

\usepackage[backend=biber, style=numeric, natbib=true, url=false, eprint=false]{biblatex}
\addbibresource{ais.bib}

\let\oldvec\vec
\renewcommand\vec{\bm}
\newcommand{\dd}{\mathrm{d}} % Euler's constant
\newcommand{\var}{\operatorname{var}}
\newcommand{\cov}{\operatorname{cov}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\ind}[1]{\mathbf{1}_{#1}}
\newcommand{\Xspace}{\mathcal{X}}
\newcommand{\Yspace}{\mathcal{Y}}
\newcommand{\risk}{R}
\newcommand{\Jac}{\mathrm{D}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\testset}{\mathcal{T}}
\newcommand{\comment}[1]{{\color{red} #1}}

\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}

\graphicspath{{./figures/}}
